Identifying and Consolidating Knowledge Engineering Requirements

Knowledge engineering is the process of creating and maintaining knowledge-producing systems. Throughout the history of computer science and AI, knowledge engineering workflows have been widely used because high-quality knowledge is assumed to be crucial for reliable intelligent agents. However, the landscape of knowledge engineering has changed, presenting four challenges: unaddressed stakeholder requirements, mismatched technologies, adoption barriers for new organizations, and misalignment with software engineering practices. In this paper, we propose to address these challenges by developing a reference architecture using a mainstream software methodology. By studying the requirements of different stakeholders and eras, we identify 23 essential quality attributes for evaluating reference architectures. We assess three candidate architectures from recent literature based on these attributes. Finally, we discuss the next steps towards a comprehensive reference architecture, including prioritizing quality attributes, integrating components with complementary strengths, and supporting missing socio-technical requirements. As this endeavor requires a collaborative effort, we invite all knowledge engineering researchers and practitioners to join us.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> section/attic/profiles.tex <==
\section{Stakeholder Profiles}
\label{sec:profiles}

To create a reference architecture, \cite{cloutier2010concept} identifies two complementary inputs (\autoref{fig:inputs}). On the one hand, the reference architecture needs to mine existing architectures for common patterns. We reviewed briefly existing architectures, and we return to them in \autoref{sec:refarch}. On the other hand, the reference architecture needs to explore the past and the future needs of its stakeholders, which are formalized as requirements. We consider four stakeholder profiles in this section: a knowledge explorer, a software developer, a data scientist, and a knowledge engineer, and derive their requirements later in this paper. For each stakeholder, we compile their needs, tooling, and corresponding patterns as a proxy for their current needs. We also describe its current pain points, as an indicator of future needs that should be included in the requirements.


\subsection{Knowledge Explorer} 


\filip{3.1 is possibly too long - see if we need to condense later}
% \subsubsection{Requirements and Use Cases}

As knowledge explorers, we consider stakeholders that access data to find (usually) small pieces of information from user-friendly interfaces~\cite{iglesias}. As such, knowledge explorers are not expected to be proficient with knowledge graphs, artificial intelligence, or even computer science. Knowledge explorers often are domain experts, e.g., in the fields of publishing, health, or e-commerce. One of the main requirements for knowledge explorers is having the ability to efficiently inspect the relational connections among entities through a user interface (e.g., a web browser), exploring and learning about different concepts.

\textbf{Present needs and tooling}
A knowledge explorer might use knowledge graphs to explore knowledge, browse answers to their questions (e.g., who won the FIFA world cup in 1994), or develop new ideas (e.g., scientific innovation by analogy). 
% \textbf{State-of-the-Art Tooling}
Knowledge explorer tasks can be supported by browsers, visualization tools, or tools for textual and faceted search. 

% \textbf{Browsers} 
The browser by Wikidata~\cite{vrandevcic2014wikidata} provides comprehensive access to the entire knowledge graph, and includes a free-text search that enables natural language entry to knowledge.\footnote{\url{https://www.wikidata.org/wiki/Q1}} The Ringgaard browser includes incoming links and improved ordering of the results, as well as a more visual representation of knowledge.\footnote{\url{https://ringgaard.com/kb/Q1}} The KGTK browser includes the same features like incoming links, search, and sorting, but it takes a step further by including profiling statistics and summaries of entities.\footnote{\url{https://kgtk.isi.edu/browser/Q1}} There exist also specialized browsers that are tailored to a domain use cases. For instance, the WeChangEd~\cite{thornton2022linking} Stories App browser displays the timeline for people including the organizations, places, and other people with which the person is associated in an interactive manner. The browser also integrates background knowledge from Wikidata and Wikipedia. DIVE~\cite{de2015dive} was developed to provide access to heritage objects from heterogeneous collections, using historical events and narratives as the context for searching, browsing, and presenting individual and groups of objects. 

% \textbf{Visualization tools} 
Several tools offer ways to visualize knowledge graphs. Neo4j itself has dozens of different visualization options for rendering graphs, presenting location information on a map, and dashboard tooling.\footnote{\url{https://neo4j.com/developer-blog/15-tools-for-visualizing-your-neo4j-graph-database/}, accessed on Oct 13, 2022.} A popular GUI for visualizing graphs is Gephi,\footnote{\url{https://gephi.org/}} which scales well to a larger set of nodes and provides a palette of algorithms for organizing the nodes and forcing them in relation to each other. CosmoGraph is a recent tool that can visualize a large set of graph nodes, scaling to millions of nodes and edges.\footnote{\url{https://cosmograph.app/}} 
The aforementioned KGTK browser includes a class visualization that shows its positioning in the overall ontology of a knowledge graph.
Google's embedding projection tool can support the visualization of various graph embeddings in an intuitive space, where node similarities are indicated by their distance in the space.\footnote{\url{https://projector.tensorflow.org/}, accessed on February 22nd, 2023.} 

% \textbf{Search} 
A variety of tools for textual and faceted search have been developed. Sindice~\cite{tummarello2007sindice} allowed search on Semantic Web documents based on IRIs and keywords that appeared in those documents. Other early influential tools like LODStats~\cite{auer2012lodstats}, Falcons~\cite{cheng2008falcons}, and Semantic Web Search Engine (SWSE)~\cite{harth2012searching}, were designed for distributed search over the LOD sources, and have been deprecated. LOTUS~\cite{ilievski2016lotus}, a follow-up faceted search based on ElasticSearch functionality, provided 32 matching and ranking combinations to billions of LOD triples available in the LOD Laundromat~\cite{beek2014lod}, but it is also not online anymore. The KGTK faceted search for Wikidata allows users to indicate textual content, language, query type, and type of matched node.\footnote{\url{https://kgtk.isi.edu/search/}} It also enables search for instances or subclasses of a certain term.

\textbf{Pain points}
The increasing set of tools for browsing, searching, and visualizing graphs provides relatively many options for exploring knowledge. Besides expressivity, knowledge exploration tools are increasingly designed to scale to a large number of nodes. A design challenge with such interfaces is that their semantics may be ambiguous, i.e., it may not be clear what is the meaning of seeing certain statements rendered in a browser~\cite{}. A more obvious challenge is that the tooling for knowledge explorers is not well-connected. In other words, there is no clear workflow that provides a gentle introduction to knowledge explorers, e.g., starting with a high-level summary of a graph to a micro-level exploration of individual nodes and knowledge statements. This observation motivates the need for research on knowledge architectures that connect the dots between individual tools to facilitate easier conceptualization by such stakeholders. A related pain point is the lack of user studies that could provide us with a deeper insight into the experience of knowledge explorers.

% Key pain points from a knowledge explorer perspective are the lack of streamed workflow from high- to micro-level, the lack of user studies, the ambiguity of interface semantics, and issues with compositionality and data quality.

% \subsubsection{KGE Reference Architecture for Knowledge Explorers}

\subsection{Software Engineer} 

% \subsubsection{Requirements and Use Cases}

% \textbf{Software developer} 

According to Wikipedia, a software engineer is ``a person who applies the principles of software engineering to design, develop, maintain, test, and evaluate computer software''.\footnote{\url{https://en.wikipedia.org/wiki/Software_engineering}, accessed on February 22nd, 2023.}  \filip{to be expanded}

\textbf{Present needs and tooling} Background knowledge may benefit software engineers in several ways. For instance, software engineering may perform content enrichment, develop recommendation techniques, or use high-level functionality for obtaining specific query results.
% \subsubsection{State-of-the-Art Tooling}
These tasks require well-abstracted data catalogs and high-level functions for the retrieval of information in a developer-friendly way. 

Content enrichment ... \filip{tbd}

Recommendation ... \filip{tbd}

\textbf{Pain points}
Software engineers can, therefore, tap into the available knowledge previously prepared by knowledge engineers. Besides more traditional applications based on content enrichment and recommendation, this is also clear from recent AI trends with models like ChatGPT that provide potentially useful responses in natural language. A key obstacle from a software engineer perspective towards a broad adoption of knowledge resources is a mismatch of assumptions and common practices, i.e., the stack of tooling and formats used by software engineers is often different from those developed by knowledge graph engineers. Further obstacles include the lack of high-level functionality, the lack of software developer-friendly documentation, and the lack of easily accessible data catalogues. 


% \subsubsection{KGE Reference Architecture for Software Developers}

\subsection{Data Scientist} 

Data scientists draw insights and build predictive models from data using various techniques, with machine learning being one of the most popular~\cite{iglesias}.
A frequent measurable goal of data scientists is to minimize failure in prediction tasks according to specific metrics, such as accuracy or precision. As the quality of the data is largely determining the quality of the developed models, data scientists may use available knowledge to enhance their training process and ultimately boost or evaluate the performance of their models.


\textbf{Present needs and tooling}
Knowledge may play different roles in a data science workflow. It may support the development of a model for a specific task (e.g., entity linking), a larger suite of tasks (e.g., analytical operations), or support benchmarking and evaluation. We descibe each of these applications in turn.


Specific data science tasks include information extraction, question answering, and link prediction.
% \subsubsection{State-of-the-Art Tooling}
A popular information extraction task is entity linking from text, which has resulted in a long list of systems, including DBpedia Spotlight~\cite{mendes2011dbpedia} and ReFinED~\cite{ayoola2022refined}. Entity linking from tables can be achieved with tooling like TabEL~\cite{bhagavatula2015tabel}. Another task is relation extraction, where the goal is to connect relations mentioned in the text to their semantic representation in background knowledge~\cite{guo2019attention}. Question answering leverages a large amount of factual, domain, or commonsense knowledge available in knowledge resources to answer open-ended questions, as exemplified by methods like QA-GNN~\cite{yasunaga2021qa} and Path Generator~\cite{wang2020connecting}.
Link prediction addresses the inherent sparsity of knowledge structures, aiming to facilitate predictive applications by methods like TransE~\cite{bordes2013translating} and RotatE~\cite{sun2019rotate}. Many of these applications rely on representation learning, i.e., translating symbolic and subsymbolic structures into embedding vectors, supported by libraries like PyTorch Geometric~\cite{fey2019fast} and PyKEEN~\cite{ali2021pykeen}. Injection of symbolic knowledge into neural (language) models has motivated tools for lexicalization and linearization of knowledge graphs, like TekGen~\cite{agarwal2020knowledge}.

% \textbf{Integrated tools and libraries} 
Integrated tools, databases, or libraries allow developers to perform a set of these operations in the same framework, avoiding the need to compose different toolkits, formats, and standards themselves. Neo4J~\cite{webber2012programmatic} facilitates a large set of graph querying and analytics operations. The Knowledge Graph ToolKit (KGTK)~\cite{ilievski2020kgtk} integrates a wide range of transformation, analytics, and data science operations in a single framework. Libraries in a variety of programming languages, like NetworkX~\cite{hagberg2008exploring} for Python, Jena~\cite{mcbride2002jena} for Java, and N3.js for Node JS,\footnote{\url{https://github.com/rdfjs/N3.js}} enable local RDF graphs to be easily loaded and queried.

% \textbf{Evaluation and audit tooling} 
GERBIL~\cite{usbeck2015gerbil} is a benchmarking tool that facilitates fair comparison of entity linking methods over a wide range of benchmarks, comparing their performance both per benchmark as well as per benchmark subsets (in-KB vs out-of-KB, for different entity types, etc.). A follow-up tool is GERBIL-QA~\cite{usbeck2019benchmarking}, which analogously measures the performance of question-answering systems. A recent tool for auditing the performance of knowledge graph completion methods is KGxBoard~\cite{widjaja2022kgxboard}, which records performance overall and per meaningful buckets, such as relation type, relation symmetry, and functionality.

\textbf{Pain points}
Existing tooling has bridged the gap between discrete symbolic knowledge and neural representations of data science tasks. Still, knowledge structures are often left out of data science mainstream research. While their promise is to provide reliable and systematic knowledge, large knowledge resources may have inconsistent ontologies~\cite{}, outdated knowledge~\cite{}, and be extremely sparse~\cite{dong}. Besides challenges with the quality of the knowledge, usage of knowledge in data science is hindered by the lack of high-level functions and easy-to-use data catalogs. Finally, there is no decision-support mechanism that can help data science practitioners use the best tool for their job.

% \subsubsection{KGE Reference Architecture for Data Scientists}

\subsection{Knowledge Engineer} 

Knowledge engineers build, maintain, and query knowledge-based systems~\cite{iglesias}. Consequently, they require efficient and easy-to-use ways to access and modify information systematically.

% \subsubsection{Requirements and Use Cases}
\textbf{Present needs and tooling}
Tools for knowledge engineers can be divided into two groups based on their intent: they support querying or contributing to knowledge artifacts.
Typical query endpoints for knowledge graphs in RDF format are SPARQL endpoints, offered by triple stores like Virtuoso~\cite{erling2009rdf} and graph databases like Graph DB.\footnote{\url{https://www.ontotext.com/products/graphdb}} To deal with issues of scalability and availability of SPARQL endpoints, Linked Data Fragments move some of the query load to the client side~\cite{verborgh2014web}. Recent popular possibilities are Neo4j's Cypher~\cite{francis2018cypher} query language and KGTK's Kypher~\cite{chalupsky2021creating} language, both of which leverage query structure analogous to SQL.

Knowledge engineers often create or modify knowledge artifacts. Small-scale expressive knowledge engineering is traditionally done with ontology editors like Protege~\cite{noy2003protege}, which focus on supporting semantic modeling. Large-scale knowledge contributions are often based on information extraction, or on crowdsourcing. An example of the latter case is Wikidata, whose knowledge engineering relies on supporting a wide community of editors with tools that ensure data quality or improve the editing experience. More recently, knowledge engineering is often done by a neural `wrapper'~\cite{bosselut2019comet} that learns how to generate knowledge or via prompt engineering~\cite{radford2019language}, which is emerging as a new discipline. 


% A knowledge engineer might contribute or edit new knowledge or provenance, perform semantic modeling and validation, infer new knowledge, or engineer a new knowledge graph.
% Key tools for knowledge engineers include ontology editors, tooling for Wikidata contributors, and knowledge construction and validation tools. 

\textbf{Pain points}
A challenge with existing querying tools is that inference at scale is still challenging. Traditional challenges with contributing to knowledge are that identity is hard to establish (which may result in duplicates) and that is-a flavors are non-trivial to distinguish~\cite{shenoy2022study}. While knowledge engineering tools support querying and modification to some extent, there is a lack of tools that support the creation of large-scale knowledge artifacts. To support better tooling for knowledge engineers, it is important to perform a wider range of user studies and standardize logging practices.

% The key pain points for knowledge engineers are that inference at scale is challenging, identity is hard to establish, different is-a flavors are difficult to distinguish, the lack of tool integration, and the lack of user studies and logging practices.

% \subsubsection{KGE Reference Architecture for Knowledge Engineers}


==> section/attic/refarch.tex <==
% \begin{appendix}

\section{Discussion: Towards a Reference Architecture for Knowledge Engineering with Knowledge Graphs}
\label{sec:refarch}

% \subsection{Knowledge engineering with knowledge graphs as a use case for data platform architectures}


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{img/KGTK Data Infrastructure.pdf}
    \caption{KGTK as a Reference Architecture for Knowledge Engineering for KGs.}
    \label{fig:kgtk_infra}
\end{figure*}


% \subsection{Analysis of specific architectures}


\subsection{A Unified Reference Architecture for KE with KGs}

The evolution of knowledge engineering and the adoption of knowledge graphs as the representation of choice.

The Semantic Web era pioneered the demonstration of business value using knowledge graphs.

But enterprise adoption has been slow, and many commercial uses deviate from canonical SW practice as defined by Berners-Lee's linked data principles.

Pace Berners-Lee, we argue this is best accomplished by applying linked data principles selectively without adherence to specific SW technologies such as RDF, SPARQL.

\textbf{Benefits}
This approach allows software engineers to perform knowledge engineering within a familiar, industry-standard framework, while benefiting from the availability within that framework of much tooling for data engineering and data science that goes considerably beyond that developed with Semantic Web stacks, for example, tools  for data observability, data curation, data governance and other DataOps elements of the mainstream data stack.

The above addresses the question of making the KE-for-KG use case more accessible to software engineers within an enterprise; what about software engineers in academic or non-profit contexts? The reference architecture is still valid, but the choice of off-the-shelf components should lean towards open-source choices. The integration of KGTK concepts within applications such as Datasette, for example, would yield the ability to easily and cheaply publish knowledge graphs based on, for example, hand-curated aggregation of open-source data or cultural heritage resources.

In addition, the KE-for-KG architecture inherits four main value propositions of other Reference Architectures: knowledge management to reuse good practices, control of complexity through standardization, common understanding of parts of the architecture, and risk mitigation by reusing known architecture patterns rather than designing new ones from scratch~\cite{cloutier2010concept}.

\subsection{Priority Ranking of KGE Requirements}
\label{sec:survey}

Previously, we indicated that the set of business/organizational goals and quality attributes presented in the previous section aims to take into account the needs and the pain point of various knowledge engineering stakeholders. Following software management practices~\cite{sangwan2007business}, the next step in the process of standardizing an infrastructure is to understand the importance (priority) of each business goal an quality attributes. As our intent is to facilitate value creation through knowledge technologies for various stakeholders, we will conduct a survey with a diverse set of KGE stakeholders, where we ask each participant to score the goals and attributes according to their relevance for them and their organization.

\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{img/survey.png}
    \caption{A snapshot of the three components of our user survey form.}
    \label{fig:survey}
\end{figure*}


% \subsubsection{Survey Design}

We will design the survey as a Google Form that consists of three sections (Figure~\ref{fig:survey}). First, we would collect general demographic information about our users: \textbf{roles} (Software engineer, Data engineer, Knowledge engineer, Data scientist,
Knowledge scientist, 
Knowledge explorer, or
Other - specify), \textbf{current location of employment} (Africa,
Americas,
Asia,
Australia, or
Europe), \textbf{application areas of interest} (E-commerce,
Digital Humanities,
Health,
Smart cities,
Library and publication,
Scientific discovery,
Finance,
Internet of Things, or
Other), 
\textbf{type of organization} (Academia,
Industry,
Government, or
Other), and \textbf{expertise with Knowledge Graphs/Knowledge Engineering} (five-point scale ranging from 1= novice user to 5=expert).
In all cases, the Other category was accompanied by a free-text input field where the user could specify an alternative value. The aspects indicated in the plural (roles and application areas of interest) allow for multiple choices to be selected. We note that the form was anonymous - we did not collect any personally identifiable information.

The second section of the form concerns the importance of each of the 22 organizational goals (B1-B22) that we identified in the previous section, by asking ``How important are the following organizational goals for knowledge graph engineering to you or your organization?''. For each of these goals, we ask the user to pick one of three options: \textit{Highly important},	\textit{Somewhat important}, and	\textit{Of low importance}. At the end of the second section, we ask participants to note any vital organizational goals for them that are missing in the survey form in a free-text field.
The third section in the form mirrors the second section for the 12 quality attributes (Q1-Q12) listed in the previous section.

% \subsubsection{Survey Participants}

When carrying out a user survey, it is essential to be deliberate about the profiles of users that can provide the most meaningful input. Prior surveys in the Semantic Web realm are rare, and when done, they have either focused on technology experts~\cite{hogan2020semantic}, or domain experts~\cite{tharani2021much}. In this paper, we take a broader view and make an attempt to understand the perspective of stakeholders belonging to a variety of roles, including Software engineer, Data engineer, Knowledge engineer, Data scientist, Knowledge scientist, and Knowledge explorer. Unlike the practice in prior work to advertise the survey in specific mailing lists, we include participants that seek to create or leverage knowledge graphs in a variety of scenarios. For this purpose, we collected participants from multiple events, including The tutorial on the Knowledge Graph Toolkit (KGTK) at AAAI'23.
    % \item \filip{TBD}
% \end{enumerate}




% \end{appendix}

==> section/attic/relatedwork.tex <==
\section{Related Work}
\label{sec:relwork}

\subsection{Architectures for Knowledge Engineering/KG Workflows}

\textbf{General architectures} CommonKADS, expert systems

\textbf{Domain-specific KG Workflows (Libraries, digital humanities, enterprise)}
A positive example of the adoption of SW technologies is the usage of Wikidata by libraries.
A systematic review of the usage of Wikidata in the discipline of Library and Information Studies (LIS)~\cite{tharani2021much} reveals Wikidata is primarily treated as a reputable and reusable knowledge base that allows libraries to connect their local metadata to a global network of metadata. In this context, Wikidata is primarily used to link authority data and improve the quality of metadata and processes. The author notes that the adoption of Wikidata has been largely driven by user-friendly tools and interfaces, as well as the quality and breadth of data. The result of this effort is apparent, as scholarly knowledge is the dominant knowledge type in Wikidata. However, the authors also caution that the incentive for prolonged adoption is important, as the effort to bring additional knowledge into libraries needs to be justified. The most salient motivation (payoff) for libraries is their discoverability and enhanced online presence when they contribute their data to Wikidata. Another positive example of adopting SW technologies with a clear return is the Amazon Product Knowledge Graph~\cite{zalmout2021all}.


\textbf{State of the Semantic Web}
While success stories of these technologies can be found among Wikidata, schema.org~\cite{guha2016schema}, and industrial Knowledge Graph~\cite{shrivastava2017bring}, Hogan~\cite{hogan2020semantic} suggests that the development of Semantic Web (SW) technologies should be driven by other research disciplines, and by practitioners and developers outside of academia. In his reflective study of the initial two decades, Hogan observes that the criticisms of SW combine human, social, technical, and economic factors. While technical concerns such as the lack of tools may be expected to be addressed, the other categories relating to incentives for adoption beyond the SW community may require a paradigm shift. 
This paper calls for action to make SW technologies accessible for outsiders and newcomers, and to work towards bridging the gap between SW and technologies that have similar goals.


\subsection{Reference Architectures for Software}

\textbf{Reference architectures as a means of driving software technology adoption}
A key artifact for use in new technology adoption within a software engineering community of practice is that of a reference architecture.
A reference architecture is a way of capturing a set of design patterns that together provide a framework to build and design software systems. Thus an architecture is a bridge between (sometimes abstract) business goals and the final (concrete) resulting software system.
Angelov et al.~\cite{angelov2009classification} define RAs as generic architecture for a class of information systems that are used as a foundation for the design of concrete architectures in this class. Bass et al.~\cite{bass2015devops} state that `a RA is a reference model mapped onto software elements (that cooperatively implement the functionality defined in the reference model) and the data that flows between them'.
RAs have several shared characteristics: they provide the highest level of abstraction, they emphasize heavily architectural qualities, their stakeholders are considered but absent from the architecture, they promote adherence to common standards, and are effective for system development and communication~\cite{ataei2022state}. Notably, while architectures capture software structures, not every structure is architectural: an architecture is an abstraction that should emphasize the attributes that are important to stakeholders~\cite{bass2022software}. 

Reference architectures are driven by two emerging trends~\cite{cloutier2010concept}. First, an increasing complexity, scope, and size of the system of interest, its context, and the organizations creating the system. Second, increasing dynamics and integration, i.e., shorter time to market, more interoperability, rapid changes, and adaptations in the field.

In \cite{bass2022software}, the authors identify thirteen uses for developing a central reference architecture.
A key aspect of reference architectures, along with related types of architectural artifacts, is that they are key to the creation of a technology strategy that drives consensus across multiple groups of stakeholders with an enterprise engaged in software application development for business purposes.
Other benefits include that RAs enable the system's quality attributes, enable early prediction of system qualities, they encode fundamental design decisions, support training of new team members, reduces system complexity, and facilitate reuse. Reference architectures provide a common lexicon and taxonomy, a common architectural vision, and modularization~\cite{cloutier2010concept}. Notably, a good architecture is necessary but not sufficient to ensure quality.


\textbf{Emerging industry architectures for data platforms}
Many RAs have been proposed in the past decades, some of which have gained wide adoption in their domains. Well known examples are CORBA for object integration through brokers~\cite{boldt95}, AUTOSAR for automotive sector~\cite{staron2021autosar}, S3 for service-oriented solutions~\cite{arsanjani2007s3}, EIRA for e-Government systems,\footnote{\url{https://joinup.ec.europa.eu/collection/european-interoperability-reference-architecture-eira/about}} and NIST's Big Data Interoperability Framework~\cite{framework2015draft}. For a comprehensive review of software RAs, we refer the reader to~\cite{garces2021three}.

The A16Z reference architecture for emerging data infrastructure and platforms is a snapshot of the current industry stack and trends that subsumes most current uses of data within and enterprise.
Description of the reference architecture's elements and workflows. Specific reference to data ingestion, transformation tooling adopted broadly by industry. See diagram from A16Z white paper in \autoref{fig:udi}.
It is noteworthy that this architecture makes no reference at all to knowledge graphs or Semantic Web concepts or products, especially given the care it takes to address specific use cases related to machine learning.

Ironically, while the field of Semantic Web puts a lot of emphasis on developing artifacts like ontologies and KGs that enable common understanding between humans and machines, it has not caught up on the idea of developing architectures that will provide a common language in which different concerns can be expressed, negotiated, and resolved among stakeholders for large, complex systems~\cite{bass2022software}.

\textbf{Methods for creating RAs/SAs}
A method to design a software architecture has been proposed by~\cite{nakagawa2011aspect}, consisting of five steps: establishing its scope, selecting and investigating information sources, performing an architectural analysis to identify architecturally significant requirements, carrying out synthesis of the reference architecture, and evaluating the architecture through surveys as well as its instantiation and use.
Typical RAs for big data usually follow a three-step lifecycle consisting of data ingestion, transformation, and serving~\cite{ataei2022state}. Their major architectural components can be roughly grouped into 1) big data management and storage, 2) data processing and application interfaces, and 3) big data infrastructure.

% \filip{the part below is moved from later section, should be incorporated}


\begin{figure*}
    \centering
    \includegraphics[width=\linewidth]{img/UDI.png}
    \caption{Unified Data Architecture from \cite{bornstein2020emerging}.}
    \label{fig:udi}
\end{figure*}



==> section/intro.tex <==
\section{Introduction}
\label{sec:intro}

Today's knowledge graphs contain a wealth of information. Possibly the most popular and largest general-domain graph, Wikidata~\cite{vrandevcic2014wikidata}, contains billions of statements for millions of notable entities, with recorded provenance and semantic constraints. Meanwhile, many other structured knowledge sources exist, some focusing on a narrow domain and others with a broad focus. These knowledge graphs found some adoption in enterprise settings~\cite{zalmout2021all}, as well as in domains like publishing and libraries~\cite{tharani2021much}.

Knowledge graphs come into existence through laborious knowledge engineering processes.
\textit{How does one engineer a knowledge graph?} Traditional knowledge engineering methods, such as CommonKADS \cite{schreiber2000knowledge}, focus heavily on knowledge elicitation from humans and are not applicable in the current socio-technical context where knowledge at scale comes from crowdsourcing, unstructured data, or neural (language) models. W3C recommendations such as the layered Semantic Web cake~\cite{hendler2009tonight} prescribe semantic components that should be used as building blocks, but it is unclear what is the engineering process to put everything together. The lack of consensus about how to approach the creation of a knowledge graph and how to represent the final knowledge product has manifested in recent alternatives to these standards, such as labeled property graphs and the Wikidata qualifier model. Bottom-up efforts~\cite{tamavsauskaite2022defining,ilievski2020kgtk} to describe the process of knowledge engineering attempt to reconcile the steps observed in practice into a joint architecture. Yet, there is a lack of consensus around a comprehensive architecture for KGE today.

In software engineering, a \textit{reference architecture (RA)} is a key artifact that drives the technology adoption within a community of practice, by capturing design patterns that together provide a flexible framework to build and design software systems. RAs drive consensus across multiple groups of stakeholders with an enterprise engaged in software application development for business purposes. Recent reports on RAs for emerging data infrastructure~\cite{bornstein2020emerging} demonstrate how the general framework of software engineering can be instantiated for AI technologies, with a particular focus on data science use cases supported by libraries like Hugging Face \cite{wolf2019huggingface}. It is noteworthy that this architecture makes no reference at all to knowledge engineering concepts or products, including knowledge graphs and the Semantic Web.
% Benefits: interoperability, reuse, ...?

Given this misalignment between knowledge engineering and software engineering practices, we deduce that practice so far
% Given that the architectures for knowledge engineering are implicit or not obviously aligned with the reference architecture for emerging software technologies, we consider the following questions: Are knowledge graph engineering processes idiosyncratic, or, alternatively, can they be mapped to such a reference architecture? While practice so far 
has assumed that knowledge engineering is an idiosyncratic process. 
Instead, we argue that it is possible, and in fact, beneficial, to work towards a reference architecture for knowledge engineering that resembles standard software engineering procedures applied in other fields like data science. We believe that this is a critical step towards the adoption of knowledge technologies by the mainstream software engineering community.


In this paper, we make the first step toward the development of a reference architecture for knowledge engineering, by identifying requirements for knowledge engineering that have arisen as a consensus across diverse stakeholders. We start with an analysis of existing knowledge engineering workflows, contrasting them with mainstream software architectures, and eliciting a methodology to bridge the gap between the two, in~\autoref{sec:relwork}. We profile four complementary stakeholder personas, each with their typical needs, corresponding tooling, and pain points as indicators for unsatisfied needs, in~\autoref{sec:profile}. Then, we take a broad historical perspective to align the stakeholder profiles into an extensive list of 8 functional requirements and 23 quality attributes in \autoref{sec:reqs}. 
In \autoref{sec:evaluation}, we select three prominent and relatively recent knowledge engineering architectures and evaluate their suitability to satisfy the identified quality attributes. We conclude the paper with a path toward a reference architecture for knowledge engineering in \autoref{sec:conclusion}.




